On Convergence of Gradient Descent Ascent: A Tight Local Analysis

Gradient Descent Ascent (GDA) methods are the mainstream algorithms for minimax optimization in generative adversarial networks (GANs). Convergence properties of GDA have drawn significant interest in the recent literature. Specifically, for $\min_{\mathbf{x}} \max_{\mathbf{y}} f(\mathbf{x};\mathbf{y})$ where $f$ is strongly-concave in $\mathbf{y}$ and possibly nonconvex in $\mathbf{x}$, (Lin et al., 2020) proved the convergence of GDA with a stepsize ratio $\eta_{\mathbf{y}}/\eta_{\mathbf{x}}=\Theta(\kappa^2)$ where $\eta_{\mathbf{x}}$ and $\eta_{\mathbf{y}}$ are the stepsizes for $\mathbf{x}$ and $\mathbf{y}$ and $\kappa$ is the condition number for $\mathbf{y}$. While this stepsize ratio suggests a slow training of the min player, practical GAN algorithms typically adopt similar stepsizes for both variables, indicating a wide gap between theoretical and empirical results. In this paper, we aim to bridge this gap by analyzing the \emph{local convergence} of general \emph{nonconvex-nonconcave} minimax problems. We demonstrate that a stepsize ratio of $\Theta(\kappa)$ is necessary and sufficient for local convergence of GDA to a Stackelberg Equilibrium, where $\kappa$ is the local condition number for $\mathbf{y}$. We prove a nearly tight convergence rate with a matching lower bound. We further extend the convergence guarantees to stochastic GDA and extra-gradient methods (EG). Finally, we conduct several numerical experiments to support our theoretical findings.

==> Sections/extension.tex <==
In this section, we extend our result to two more general settings: 1) the function is nearly quadratic and 2) the gradient oracle is stochastic.
We will assume $s=1$, i.e., the matrix $M$ is diagonalizable throughout this section and leave the case it is not to future work.% We will keep $r=2\ky$ and our analysis can be directly extended to any $r\ge 2\ky$.
\subsection{Nearly quadratic functions}
Suppose $f:\R^n\times\R^m\to \R$ belongs to the function class of interest. In this section, we assume that $f(\vx;\cdot)$ is $\mu$-strongly concave for any fixed $\vx$ and $f(\cdot;\cdot)$ is ${L}$-smooth as in Section~\ref{sec:theory}. Similar to Section~\ref{sec:42}, we assume $\Phi(\cdot):=\max_{\vy}f(\cdot;\vy)$ is strictly convex through this section. Let $\vx^\ast$ be its unique global minimum and $\vy^\ast:=\argmax_{\vy}f(\vx^\ast;\vy)$. Assume that $f$ is twice continuously differentiable, which implies the Hessian at every point exists and is symmetric. We denote the Hessian at the optimal point $(\vx^\ast,\vy^\ast)$ as
	\begin{align*}
	 \begin{pmatrix}
	C & B \\ B^\top & -A
	\end{pmatrix} :=\nabla^2 f(\vx^\ast;\vy^\ast),  
	\end{align*}
	i.e., $C:=\nabla^2_{\vx\vx}f(\vx^\ast;\vy^\ast)$, $B:=\nabla^2_{\vx\vy}f(\vx^\ast;\vy^\ast)$, and $A:=-\nabla^2_{\vy\vy}f(\vx^\ast;\vy^\ast)$.
	Also define
	\begin{align*}
	M  := \begin{pmatrix}
	-C & -B \\ r B^\top & -r A
	\end{pmatrix} .
	\end{align*}
	We know $A,C$ are symmetric and $\mu I \le A\le {L}I$, $\|B\|_2, \|C\|_2\le {L}$. Also define $\mux=\min\left\{L,\lambda_{\min}(C+BA^{-1}B^\top)\right\}>0$ as $\Phi$ is strictly convex. We assume $f$ is nearly quadratic: the Hessian of $f$ satisfies the following assumption.
	\begin{assumption}
		There exist some nonnegative scalars $\Delta_{\vx\vx},\Delta_{\vx\vy},\Delta_{\vy\vy}\ge 0$ such that the Hessian of $f$ at every point $(\vx,\vy)$ satisfies
	\begin{align*}
	\|\nabla^2_{\vx\vx}f(\vx;\vy)-C\|_2\le& \Delta_{\vx\vx},\\
	\|\nabla^2_{\vx\vy}f(\vx;\vy)-B\|_2\le& \Delta_{\vx\vy},\\
	\|\nabla^2_{\vy\vy}f(\vx;\vy)+A\|_2\le& \Delta_{\vy\vy}.
	\end{align*} 
	\label{assumption:near_quad}
	\end{assumption}
Let $\Delta_r := \Delta_{\vx\vx}+\left(r+1\right)\Delta_{\vx\vy}+r \Delta_{\vy\vy}$. In the following theorem, we show that if $\Delta_{r}$ is small enough, i.e., the function is nearly quadratic, GDA has a linear convergence rate. 
\begin{theorem}
	\label{thm:conv_general}
 Suppose $M=P^{-1
	}\Lambda P$ is diagonizable. Let $C_P=\norm{P}_2\norm{P^{-1}}_2$. Choose $\etax=\frac{1}{2r L}$ and $\etay=\frac{1}{2L}$ where $r\ge 2\ky$. If $\Delta_{r}\le \frac{\mux}{8 C_P}$, we have  
	\begin{align*}
	\|\vz^T-\vz^\ast\|_2\le C_P\norm{\vz^0-\vz^\ast}_2\left(1-\frac{1}{16r\kx}\right)^T.
	\end{align*}
	It means the gradient complexity of achieving an error less than $\epsilon$ is\begin{align*}
	\cO\left(r\kx\log\left(\frac{C_P\norm{\vz^0-\vz^\ast}_2}{\epsilon}\right)\right).
	\end{align*}
\end{theorem}
%\haochuan{Can we do nondiagonalizable $M$?}
Note that given any general nonconvex-strongly-concave function $f$, we know that Assumption~\ref{assumption:near_quad} holds within a sufficiently small neighborhood around some local stationary point. Therefore, Theorem~\ref{thm:conv_general} can be viewed as a local convergence theory for general NC-SC functions. Formally, it leads to the following theorem.
\begin{theorem}
\label{cor:local}
For a NC-SC smooth function $f(\vx;\vy)$, Let $\vx^\ast$ be a strict stationary point of its primal function $\Phi(\vx)=\max_{\vy}f(\vx;\vy)$ and $\vy^\ast=\argmax_{\vy}f(\vx^\ast;\vy)$. Then if $(\vx^0,\vy^0)$ is initialized within a sufficient neighborhood around $(\vx^\ast,\vy^\ast)$, GDA with $\etax=\frac{1}{2r L}$ and $\etay=\frac{1}{2L}$ where $r\ge 2\ky$ converges to $(\vx^\ast,\vy^\ast)$ locally at a linear rate.
\end{theorem}

%----------------------------------------------------

%----------------------------------------------------

\subsection{Stochastic gradient oracle}
Now we extend our result to mini-batch stochastic gradient descent-ascent (SGDA) for quadratic functions with a stochastic oracle. The analysis below can be possibly extended to nearly quadratic functions and we leave this to future work. The function $f$ takes the form and assumptions as in Section~\ref{sec:pre}. However, only a stochastic estimate of the gradient is available to the algorithm.
The mini-batch SGDA update rule with batch size $S$ can be written as
\begin{align*}
\vx^{k+1} &= \vx^k -\etax \nabla_{\vx} f(\vx^k;\vy^k)-\etax\tfrac{1}{S}\textstyle\sum_{i=1}^{S}\vxi^{\vx}_{k,i}\\
\vy^{k+1} &= \vy^k +\etay \nabla_{\vy} f(\vx^k;\vy^k)+\etay\tfrac{1}{S}\textstyle\sum_{i=1}^{S}\vxi^{\vy}_{k,i},
\end{align*}
where for each fixed $k$, the noises $\left\{\left(\vxi^{\vx}_{k,i},\vxi^{\vy}_{k,i}\right)\right\}_{i=1}^S$ are i.i.d. sampled from some unknown distribution. We impose the standard assumption of zero mean and bounded variance on the noises:
\begin{assumption}
    We assume $\E[\vxi^{\vx}_{k,i}]=\0$, $\E[\vxi^{\vy}_{k,i}]=\0$, $\E[\|\vxi^{\vx}_{k,i}\|_2^2]\le \sigma_{\vx}^2$, and $\E[\|\vxi^{\vy}_{k,i}\|_2^2]\le \sigma_{\vy}^2$ for some $\sigma_{\vx},\sigma_{\vy}\ge 0$.
\end{assumption}

 We also denote 
\begin{align*}
\vxi_k=	\begin{pmatrix}
-\frac{1}{S}\sum_{i=1}^{S}\vxi^{\vx}_{k,i} \\ \frac{r}{S}\sum_{i=1}^{S}\vxi^{\vy}_{k,i}
\end{pmatrix}.
\end{align*}
We know $\E[\norm{\vxi_k}_2^2]\le  ({\sigma_{\vx}^2+r^2\sigma_{\vy}^2})/S=: \sigma_r^2/S$. The following theorem establishes a convergence result for mini-batch SGDA. 
\begin{theorem}
	\label{thm:conv_general_sgda}
	We use the same parameters as in Theorem~\ref{thm:conv_general}. Suppose $M=P^{-1}\Lambda P$ is diagonizable. We have  
	\begin{align*}
	\E[\|\vz^T-\vz^\ast\|_2^2]\le& C_P^2\norm{\vz^0-\vz^\ast}_2^2\left(1-\frac{1}{16\kappa\kx}\right)^{2T}\\&+\frac{2\kx C_P^2\sigma^2_{r}}{rL^2 S}.
	\end{align*}
	 It means the gradient complexity of achieving $	\E[\|\vz^T-\vz^\ast\|_2^2]\le\epsilon^2$ is\begin{align*}
	\cO\left(r\kx\log\left(\frac{C_P\norm{\vz^0-\vz^\ast}_2}{\epsilon}\right)\max\left\{1,\frac{\kx C_P^2\sigma^2_{r}}{rL^2 \epsilon^2}\right\}\right).
	\end{align*}
\end{theorem}
Remark that if $\max\{\sigma_{\vx},\sigma_{\vy}\}=\cO(1)$, we know $\sigma_{r}^2=\cO(r^2)$ and the above complexity is 
\begin{align*}
\Tilde{\cO}\left(\frac{r^2\kx^2}{\epsilon^2}\right).
\end{align*}




==> Sections/theory.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
  \centering

  \begin{tabular}{cccc}
    \toprule
settings & GDA with $\mux>0$ & GDA with $\mux=0$ & SGDA with $\mux>0$  \\
\midrule
     %$r\le \kappa$& $\infty$ & $\infty$ & $\infty$ \\
     %\midrule
     $r=2\kappa$ (Ours)& $\Tilde{\cO}\left(\kappa\kx\right)$ & $\Tilde{\cO}\left(\kappa/\epsilon\right)$ & $\Tilde{\cO}\left({\kappa^2\kx^2}/{\epsilon^2}\right)$ \\
     \midrule
     $r=\Theta(\kappa^2)$ \citep{lin2020gradient}
     & $\Tilde{\cO}\left(\kappa^2\kx\right)$ & $\Tilde{\cO}\left(\kappa^2/\epsilon\right)$ & $\Tilde{\cO}\left({\kappa^4\kx^2}/{\epsilon^2}\right)$ \\
    \bottomrule
  \end{tabular}
  \caption{Gradient complexity upper bounds of (S)GDA with $\etax=\Theta(1/r L)$ and $\etay=\Theta(1/L)$ on quadratic NC-SC functions to achieve $\norm{\vx-\vx^\ast}_2^2+\norm{\vy-\vy^\ast}_2^2\le\epsilon^2$ for $\mux>0$ or $\Phi(\vx)-\Phi(\vx^\ast)\le \epsilon$ when $\mux=0$. Here we only show the dependence on $\kappa,\kx,\epsilon$ and also hide logarithmic factors in $\Tilde{\cO}(\cdot)$.}
  \label{tab:complexity}
\end{table*}

\paragraph{Overview of results.}
In this section, we provide our convergence results of GDA on quadratic functions. We first show that to ensure convergence, the stepsize ratio $r$ must be at least $\Omega(\kappa)$ in Section~\ref{sec:lower_bound_ratio}. Then in Section~\ref{sec:42}, given any $r\ge 2\kappa$, we establish a linear convergence result when $\mux>0$, i.e., the primal function $\Phi$ is strongly convex. Then we also analyze the setting when $\mux=0$ in Section~\ref{sec:mux_zero}. 
The gradient complexity bounds for $r=2\kappa$ and $r=\Theta(\kappa^2)$ are summarized in Table~\ref{tab:complexity}, where we choose these two stepsize ratios to present because 1) $r=2\kappa$ is our optimal choice as all the upper bounds increase for a larger $r$; and 2) $r=\Theta(\kappa^2)$ is the choice in~\citep{lin2020gradient} which we want to compare our result with. As we can see from the table, the bound of $r=2\kappa$ is $\Tilde{\Theta}(\kappa)$ times tighter than that of $r=\Theta(\kappa^2)$ for GDA and even $\Tilde{\Theta}(\kappa^2)$ times tighter for SGDA.

\subsection{A lower bound of the stepsize ratio}
\label{sec:lower_bound_ratio}

To start with, we show that for unconstrained NC-SC minimax optimization problems, the stepsize ratio $r$ of GDA must be at least $\Omega(\kappa)$ to ensure convergence. Formally, we have the following theorem:
\begin{theorem}
	\label{thm:lower_bound}
	For any given $L,\mu>0$ and $0\le \mux\le L$ such that $\ky=L/\mu\ge 2$, there exists a function $f$ satisfying Assumption~\ref{assumption:quadratic} and $C+BA^{-1}B^\top\ge \mux I$ such that if choosing a stepsize ratio $r\le \kappa$, the GDA algorithm does not converge for all initial points irrespective of any choice of positive stepsize $\etax$.
\end{theorem}
Note that Theorem~\ref{thm:lower_bound} is also a lower bound of stepsize ratio for the general NC-SC function class as the quadratic function class subsumes the general one. With this lower bound, we will always choose a stepsize ratio at least linear in $\ky$.

\subsection{Linear convergence when $\mux>0$}
\label{sec:42}
Now we show that a stepsize ratio, at least linear in $\kappa$, suffices to guarantee convergence of GDA when $\mux>0$. 
We will bound $\rho<1$ to prove the linear convergence. To obtain such a bound of $\rho$, we need to analyze the spectral properties of $M$. Informally, through fine-grained analysis, we can show that if $\mux>0$ and $r>\ky$, every eigenvalue $\lambda$ of $M$ has a strictly negative real part. Moreover, the angle between the complex number $\lambda$ and the real line in the complex plane is bounded by some $\theta<\pi/2$. Therefore, when $\etax$ is small enough, $1+\etax \lambda$ will lie strictly inside the unit circle which implies $\rho<1$.

Then we can obtain the following convergence result. Note that since there is a unique optimal point $\vz^\ast$, we use the distance $\norm{\vz^T-\vz^\ast}_2$ as the performance measure instead of the notion of approximate stationary points used in \citep{lin2020gradient}.

\begin{theorem}
	Let $M=P^{-1}J P$ be its Jordan decomposition. Define $C_P=\|P\|_2\|P^{-1}\|_2$ as the condition number of $P$ and $s$ be the size of the largest Jordan block in $J$.
	Under Assumption~\ref{assumption:quadratic}, choosing $\etax=\frac{1}{2rL}$ and $\etay=\frac{1}{2L}$ with $r\ge 2\ky$ and assuming $\mux>0$, we have 
	\begin{align*}
	\|\vz^T \! - \! \vz^\ast\|_2 \! \le \!  sC_P \! \norm{\vz^0 \! - \! \vz^\ast}_2 \! T^{s-1} \! \left(1 \! - \! \frac{1}{16r\kx}\right)^{T-s+1},
	\end{align*}
% 	\haochuan{overfull}
	 which means the gradient complexity of achieving $	\|\vz^T-\vz^\ast\|_2\le\epsilon$ is\begin{align*}
\cO\left(sr\kx \log\left(\frac{sr\kx C_P\norm{\vz^0-\vz^\ast}_2}{\epsilon}\right)\right).
	\end{align*}
	\label{thm:converence_nond_1}
\end{theorem}

The gradient complexity  has a factor of $s$ which could be proportional to the dimension $d=m+n$ in the worst case but is usually very small. When $s=1$, i.e., $M$ is diagonalizable, we can actually slightly improve the complexity to $$\cO\left(r\kx\log\left(C_P\norm{\vz^0-\vz^\ast}_2/\epsilon\right)\right).$$ 

Ignoring $s$ and the log factor, the complexity is $\Tilde{\cO}(r\kx)$ which scales linearly in $r$ when $r\ge 2\ky$. So choosing $r=2\ky$ results in the best complexity bound of $\Tilde{\cO}(\ky\kx)$. This rate significantly improves upon the state-of-the-art rate, $\Tilde{\cO}(\ky^2\kx)$, of choosing $r=\Theta(\ky^2)$ as in \citep{lin2020gradient}.

Note that the condition number of the primal function $\Phi$ is $\kx(\kappa+1)$. Therefore, the $\Tilde{\cO}(\kappa\kx)$ gradient complexity for $r=2\ky$ is nearly the same as the iteration complexity of running gradient descent directly on $\Phi$ although we do not really have access to its value and gradient!


\iffalse
\subsubsection{Lower bound}
\haochuan{Currently we can show a tight lower bound only for the case $r=\Theta(\ky)$, we can not get a matching lower bound for \citep{lin2020gradient}'s stepsizes}
Now we show that the above complexity of $\Tilde{\cO}(\ky\kx)$ for the best stepsize ratio choice of $r=2\ky$ is tight in terms of dependence on $\kx$, $\ky$, and $\epsilon$. Formally, we prove the following lower bound

\begin{theorem}
 For any given $L,\mu>0$ and $0\le \mux\le L$ such that $\ky=L/\mu>4$, there exists a function $f$ satisfying Assumption~\ref{assumption:quadratic} and $C+BA^{-1}B^\top\ge \mux I$ such that GDA with a stepsize ratio $r\ge 2\ky$ can not achieve $\norm{\vz^T-\vz^\ast}_2\le \epsilon$ for some intial point $\vx^0$ until 
 \begin{align*}
     T = \Omega\left(\ky\kx\log\left(\frac{\norm{\vz^0-\vz^\ast}_2}{\epsilon}\right)\right).
 \end{align*}
 \label{lower_bound_gda}
\end{theorem}
This lower matches our upper bound for $r=\Theta(\ky)$ if ignoring $s$ and the log factor.
\fi

\subsection{Convergence when $\mux=0$}
\label{sec:mux_zero}
Now we analyze the case $\mux=0$. In this case, the previous spectral analysis can only obtain $\rho\le 1$ which itself is not sufficient to show convergence. Besides that, one also has to show the arithmetic multiplicity and geometric multiplicity of $0$ as an eigenvalue of $M$ are equal, i.e., $0$ is a regular eigenvalue. However, such analysis for $M$, a quite general block matrix, is very hard if not impossible.

We bypass this issue by adding a $\frac{\delta}{2}\norm{\vx}_2^2$ term to $\Phi$ to make it $\delta$ strongly convex, where $0<\delta\le L$ is a small scalar to be specified later. Then we can use the above analysis in Section~\ref{sec:42} on $\Phi(\vx)+\frac{\delta}{2} \norm{\vx}_2^2$. Formally, define
\begin{align*}
    f_\delta(\vx;\vy):=f(\vx;\vy)+\frac{\delta}{2} \norm{\vx}_2^2.
\end{align*}
We have
\begin{align*}
    \Phi_\delta(\vx):=\max_{\vy}f_\delta(\vx;\vy)=\Phi(\vx)+\frac{\delta}{2} \norm{\vx}_2^2.
\end{align*}
Let $\vx_\delta^\ast :=\argmin_{\vx} \Phi_\delta(\vx)$ and $\vy_\delta^\ast:=\argmin_{\vy} f(\vx_\delta^\ast;\vy)$. Also denote $\vz_\delta^\ast:=(\vx_\delta^\ast,\vy_\delta^\ast)$. Then we know that GDA applied on $f_\delta$ converges to $\vx_\delta^\ast$ at a linear rate. It is also easy to show that $\vx_\delta^\ast$ is an approximately optimal point: $ \Phi(\vx_\delta^\ast)-\Phi(\vx^\ast)\le \frac{\delta}{2}\norm{\vx^\ast}_2^2.$ Define 
\begin{align*}
    M_{\delta}=\begin{pmatrix}
-C-\delta & -B\\
r B^\top & -r A
\end{pmatrix}.
\end{align*}
we obtain the following convergence result:
\begin{theorem}
 Let $R$ be an estimated upper bound of $\norm{\vx^\ast}_2$. Choose $\delta=\epsilon/R^2$ and assume $\epsilon$ is small enough such that $\delta\le L$. 
	Let $M_\delta=P^{-1}J P$ be its Jordan decomposition. Define $C_{P}=\|P\|_2\|P^{-1}\|_2$ be the condition number of $P$ and $s$ be the size of the largest Jordan block in $J$.
	Applying GDA on $f_\delta$ with $\etax=\frac{1}{4r L}$ and $\etay=\frac{1}{4L}$ where $r\ge 2\ky$, under Assumption~\ref{assumption:quadratic}, we have \begin{align*}
	&\Phi(\vx^T)-\Phi(\vx^\ast)\le \epsilon/2\\
	&+ \,(\kappa+1)L s^2C_P^2\norm{\vz^0-\vz_\delta^\ast}_2^2T^{2(s-1)}\left(1-\frac{\epsilon}{32r L R^2}\right)^{2(T-s+1)}.
	\end{align*}
	 Therefore the gradient complexity of achieving $\Phi(\vx^T)-\Phi(\vx^\ast)\le \epsilon$ is \begin{align*}
\cO\left(\frac{sr LR^2}{\epsilon} \log\left(\frac{sr LR^2 C_P\norm{\vz^0-\vz_\delta^\ast}_2}{\epsilon}\right)\right).
	\end{align*}
	\label{thm:converence_nond_nonstrong}
\end{theorem}
Assuming $s=\cO(1)$ and ignoring the log factor, choosing $r=2\ky$, the complexity of $\Tilde{\cO}(\kappa L/\epsilon)$ is again the same as the iteration complexity of gradient descent directly on $\Phi$ although we do not have access to its gradient.


